SCNode: Spatial and Contextual Coordinates for Graph Representation Learning

Effective node representation lies at the heart of Graph Neural Networks (GNNs), as it directly impacts their ability to perform downstream tasks such as node classification and link prediction. Most existing GNNs, particularly message passing graph neural networks, rely on neighborhood aggregation to iteratively compute node embeddings. While powerful, this paradigm suffers from well-known limitations of oversquashing, oversmoothing, and underreaching that degrade representation quality. More critically, MPGNNs often assume homophily, where connected nodes share similar features or labels, leading to poor generalization in heterophilic graphs where this assumption breaks down. To address these challenges, we propose \textit{SCNode}, a \textit{Spatial-Contextual Node Embedding} framework designed to perform consistently well in both homophilic and heterophilic settings. SCNode integrates spatial and contextual information, yielding node embeddings that are not only more discriminative but also structurally aware. Our approach introduces new homophily matrices for understanding class interactions and tendencies. Extensive experiments on benchmark datasets show that SCNode achieves superior performance over conventional GNN models, demonstrating its robustness and adaptability in diverse graph structures.

==> figures/mainfig.tex <==
\begin{figure}[t]
\begin{subfigure}{.4\textwidth}
  \centering 
  % include first image
   \includegraphics[width=.8\linewidth]{figures/directed2.eps}  
\end{subfigure} \hspace{1cm}
\begin{subfigure}{.4\textwidth}
  \centering 
  \includegraphics[width=\linewidth]{figures/landmark.pdf} 
\end{subfigure}
%\vspace{-.5cm}
 \caption{\footnotesize In the figure left, we see $1$-neighborhood of the central node $u$. As the graph is directed, we obtain two feature vectors, $\vec{\alpha}_{1i}(u)=[\textcolor{red}{2} \ \textcolor{teal}{1} \ \textcolor{blue}{3}]$ for incoming and $\vec{\alpha}_{1o}(u)=[\textcolor{red}{2} \ \textcolor{teal}{4} \ \textcolor{blue}{2}]$ for outgoing nodes where colored numbers represent their class. In the figure right, we see node embeddings of a graph $\G$ with $3$ node classes in the latent space $\R^n$, and their clusters $\Z_1,\Z_2,\Z_3$.  $\xi_1,\xi_2,\xi_3$ represents cluster landmarks as colored $\triangle$s. The distances between the node embedding $\X(u)$ and the landmarks give the domain feature vector $\vec{\beta}(u)=[\textcolor{red}{d_1} \  \textcolor{teal}{d_2} \ \textcolor{blue}{d_3}]$.  \label{fig:features}}
\end{figure}

==> tables/improvements.tex <==
\begin{table*}[t]
    \caption{SCNode improvements on GNN models where we replace initial node embeddings with SCNode embeddings. \label{tab:GNN2}}
    
    
    \centering
    \resizebox{0.5\linewidth}{!}{
\begin{tabular}{ccc|cc|cc|cc||cc|cc|cc|cc}
%\toprule
&\multicolumn{8}{c}{\textbf{CORA}}&\multicolumn{8}{c}{\textbf{TEXAS}} \\
 \cmidrule(lr){2-9} \cmidrule(lr){10-17}
       \textbf{Epoch} &                  \textbf{GCN} & $\textbf{GCN-CC}$ & \textbf{GSage} & $\textbf{GSage-CC}$ & \textbf{GAT} & $\textbf{GAT-CC}$ &\textbf{LINKX} & \textbf{LINKX-CC} &\textbf{GCN} & $\textbf{GCN-CC}$ & \textbf{GSage} & $\textbf{GSage-CC}$ & \textbf{GAT} & $\textbf{GAT-CC}$ &\textbf{LINKX} & \textbf{LINKX-CC} \\
     %  \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
                          \midrule
50                   &    83.70     &    84.71      &   83.50       &  84.71        & 84.71  &  74.85 &  79.45 & 87.32 &   54.05      &    72.97     &   70.27       &  81.08        & 56.76  &  72.97  & 64.86& 83.78    \\ 
100                    &  82.90        &  86.92        &   83.70       &  88.13        & 83.30 &  81.49& 75.23 & 87.93 &   59.46     &    81.08      &   72.97       &  83.78        & 56.76  &  59.46  &59.46 &  89.19    \\ 
150                   &    82.49      &    88.13      &   84.10      &  88.93       & 82.90  &  85.31 & 72.64 & 89.94 &   51.35      &    75.68     &   75.68       &  86.48        & 54.05  &  70.27  & 62.16 &  94.59  \\ 
200                    &  81.69        &  88.93       &   83.10       &  90.95        & 81.69 &  87.32& 70.02  & 86.32 &  48.65     &    70.27      &   78.38       &  89.91        & 51.35  &  67.57   & 56.76 &  89.19   \\ 
\bottomrule
\end{tabular}
    }
    % \vskip -0.1in
\end{table*}

==> tables/ogbresults.tex <==



==> tables/wisconsinhomophily.tex <==
\begin{table}[h]
    \centering
    \caption{Spatial homophily matrix for WISCONSIN dataset. Further homophily matrices are given in \Cref{sec:heterophily_metrics}.}
    \label{tab:wis_hom_matrix1}
    \resizebox{0.5\linewidth}{!}{
    \begin{tabular}{cccccc}
        \multicolumn{6}{c}{\textbf{SCNode Spatial-1 Homophily Matrix}}\\
        \toprule
        & $\mathcal{C}_1$ & $\Cbold_2$ & $\Cbold_3$ & $\Cbold_4$ & $\Cbold_5$ \\
        \midrule
        % $\Cbold_1$ & \textbf{0.33} & 0.000 & 0.00 & 0.33 & 0.33 \\
        $\Cbold_2$ & 0.0 & 0.22 & \textbf{0.60} & 0.18 & 0.00 \\
        $\Cbold_3$ & 0.00 & \textbf{0.55} & 0.23 & 0.14 & 0.08 \\
        $\Cbold_4$ & 0.04 & 0.27 & \textbf{0.47} & 0.07 & 0.15 \\
        $\Cbold_5$ & 0.15 & 0.04 & \textbf{0.40} & 0.20 & 0.22 \\
        \bottomrule
    \end{tabular}}
\end{table}
